PhenoAuth: A Novel PUF-Phenotype-based Authentication Protocol for IoT Devices

Physical Unclonable Functions (PUFs) have been shown to be a highly promising solution for enabling high security systems tailored for low-power devices. Commonly, PUFs are utilised to generate cryptographic keys on-the-fly, replacing the need to store keys in vulnerable, non-volatile memories. Due to the physical nature of PUFs, environmental variations cause noise, manifesting themselves as errors which are apparent in the initial PUF measurements. This necessitates expensive active error correction techniques which can run counter to the goal of lightweight security. ML-based techniques for authenticating noisy PUF measurements were explored as an alternative to error correction techniques, bringing about the concept of a PUF Phenotype, where PUF identity is considered as a structure agnostic representation of the PUF, with relevant noise encoding. This work proposes a full noise-tolerant authentication protocol based on the PUF Phenotype concept and methodology for an Internet-of-Things (IoT) network, demonstrating mutual authentication and forward secrecy in a setting suitable for device-to-device communication. Upon conducting security and performance analyses, it is evident that our proposed scheme demonstrates resilience against various attacks compared to the currently existing PUF protocols.

==> figures/authentication.tex <==
\begin{mdframed}
% \fbox{
\begin{adjustbox}{max width=1.1\textwidth, max height=1\textheight}
\pseudocode[colspace=-0.47\textwidth,width=\linewidth]{
    \pcbox{\textbf{Verifier(Gateway)} \mid k_{i}} \< \< \pcbox{\textbf{Device}_{i}\mid \textbf{C}_{i}} \\[0.1\baselineskip ][\hline] 
    \<\< \\[-0.5\baselineskip ]
        \<\< \textbf{Read}(C_{i})\\
        \<\< R_{i} \gets DPUF(C_{i});k_{i}\gets KDF(R_{i})\\
        \<\< C_{d}\sample TRNG\\
        \<\< r_{d}\gets DPUF_{Dev_{i}}(C_{d})\\
        \<\< \alpha \gets AEAD.Enc(k_{i},r_{d},C_{d},t_{d})\\
    \< \sendmessageleft*{\pcbox{\boldsymbol{M_{1}}: \{Dev_{i},\alpha\}}} \< \\
    \textbf{Find:} Dev_{i},\textbf{check:} t_{d} \< \< \\
    \textbf{Load:} (k_{i},DPAN_{s}) \< \< \\
    \{r_{d},C_{d}\} \gets AEAD.Dec(k_{i},\alpha) \< \< \\
    PD_{i}\gets IMGen(r_{d}) \< \< \\
    (g_{i},X_{D_{i}}) \gets DPAN_{s}(PD_{i})  \< \< \\
    \textbf{if}\ g_{i}==Dev_{i}\ \textbf{and}\ X_{D_{i}}\geq \tau\  \textbf{then}\< \< \\
            \{  \< \< \\
            \quad C_{s}\gets TRNG  \< \< \\
            \quad r_{s} \gets DPUF_{s}(C_{s}) \< \< \\
            \quad \beta\gets AEAD.Enc(k_{i},C_{s},r_{s},Auth\_OK,C_{d},t_{s}) \< \< \\
            \} \< \< \\
    \ \textbf{else abort}\< \<\\
     \sendmessageright*{\pcbox{\boldsymbol{M_{2}}: \{Auth\_{OK},\beta,C_{s}\}}} \< \< \\
    \<\< (Auth_{OK},r_{s},C_{s})\gets AEAD.Dec(\beta) \\
    \<\< PS_{i}\gets IMGEN(r_{s_{i}})\\
    \<\< z,X_{S_{i}}\gets DPAN_{D}(PS_{i})\\
    \<\< \textbf{if}\ (\hat{z}==True)\ \textbf{and}\ X_{D_{i}}\geq \tau\  \textbf{then}\\
    \<\< \quad Accept\ \\
    \<\< \quad C_{i+1}\gets TRNG\ \\
    \<\< \quad r_{i+1}\gets DPUF(C_{i+1}) \\
    \<\< \quad k_{i+1}\gets KDF(r_{i+1}) \\
    \<\< \quad \gamma\gets AEAD.Enc(k_{i},C_{s}+1,\\
    \<\< Update\_OK,t_{d}^{'},k_{i+1})\\
    \<\< \quad \textbf{Store}\ C_{i+1} \\
    \<\< \textbf{else abort}\\
    \< \sendmessageleft*{\pcbox{\boldsymbol{M_{3}}: \{Update\_OK,\gamma\}}} \< \\
    \{k_{i+1},t_{d}^{'}\}\gets AEAD.Dec(k_{i},\gamma)\< \<\\
    \textbf{Check}\ t_{d}^{'}, C_{s} \< \<\\
    \textbf{Store}\ k_{i+1}\< \<\\
}
\end{adjustbox}
% }
\end{mdframed}

% C_{s}+1 as counter, change it to session ID (sid)

==> figures/authentication_new.tex <==
\begin{mdframed}
% \fbox{
\begin{adjustbox}{max width=1.1\textwidth, max height=1\textheight}
\pseudocode[colspace=-0.43\textwidth,width=\linewidth]{
    \pcbox{\textbf{Verifier(Gateway)}} \< \< \pcbox{\textbf{Device}_{i}\mid \textbf{C}_{i} , R_{d} \oplus R_{s}} \\[0.1\baselineskip ][\hline] 
    \<\< \\[-0.5\baselineskip ]
        \<\< \textbf{Read}\ (C_i,R_d\oplus R_s)\\
        \<\< R_{d} \gets DPUF_{dev}(C_{i})\\
        \<\< K\gets KDF(R_d)\\
        \<\< C_{i+1}\sample TRNG\\
    \< \sendmessageleft*{\pcbox{\boldsymbol{M_{1}}: \{Dev_{i},C_i,C_{i+1},R_d\oplus R_s\}}} \< \\
        R_{s} \gets DPUF_{s}(C_{i})\<\<\\
        R_d \gets (R_{d}\oplus R_{s})\oplus R_s\<\<\\
        PD_{i}\gets IMGen(R_{d}) \< \< \\
        (g_{i},X_{D_{i}}) \gets DPAN_{s}(PD_{i})  \< \< \\
        \textbf{if}\ g_{i}==Dev_{i}\ \textbf{and}\ X_{D_{i}}\geq \tau\  \textbf{then}\< \< \\
            \{  \< \< \\
            \quad K\gets KDF(R_d) \<\<\\
            \quad R_{s}^{'} \gets DPUF_{s}(C_{i+1}) \< \< \\
            \} \< \< \\
        \ \textbf{else abort}\< \<\\
    \< \sendmessageright*{\pcbox{\boldsymbol{M_{2}}: \{Auth\_OK,R_s\oplus R_s^{'}\}}} \< \\
        \<\< R_{s}^{'} \gets (R_{s}\oplus R_{s}^{'})\oplus R_s\\
        \<\< PS_{i}\gets IMGEN(R_{s}^{'})\\
        \<\< z,X_{S}\gets DPAN_{D}(PS_{i})\\
        \<\< \textbf{if}\ (\hat{z}==True)\ \textbf{and}\ X_{D_{i}}\geq \tau\  \textbf{then}\\
            \<\< \quad R_{d}^{'} \gets DPUF_{dev}(C_{i+1})\\
            \<\< \quad \textbf{Store}\ C_{i+1}, R_{d}^{'}\oplus R_{s}^{'} \\
        \<\< \textbf{else abort}\\
}
\end{adjustbox}
% }
\end{mdframed}

% One concern is that if the adversary can have access to the dram PUF and NVM, then he can read out the responses $R_{d}$

==> figures/enrollment.tex <==
\begin{mdframed}
% \fbox{
\begin{adjustbox}{max width=1.1\textwidth, max height=1\textheight}
\pseudocode[colspace=-0.3\textwidth,width=\linewidth]{
    \pcbox{\textbf{Verifier}(\ e.g.\ \textbf{Server/\ Device}_{j})} \< \< \pcbox{\textbf{Prover}(\ e.g.\ \textbf{Device}_{i})} \\[0.1\baselineskip ][\hline] 
    \<\< \\[-0.5\baselineskip ]
    \< \sendmessageleft*{\pcbox{\boldsymbol{M_{0}}: \{Dev_{i},Auth_{init}\}}} \< \\
        C_{patterns}\gets \{0xFF,0x00,0x55\} \< \< \\
        C_{i}\sample TRNG\\
        X_{s}\gets DPUF_{s}(C_{patterns}) \< \< \\
     \sendmessageright*{\pcbox{\boldsymbol{M_{1}}: \{X_{s},C_{i},C_{patterns},Server_{id}\}}} \<\< \\
        \<\< R_i \gets DPUF_{dev}(C_i)\\
        \<\< k_{i} \gets KDF(R_{i})\\
        \<\< X_d\gets DPUF_{dev}(C_{pattern})\\
        \<\< DPAN_d \gets Train(X_{s},Server_{id})\\
        \<\< \textbf{Store}\ {C_{i},DPAN_{d}}  \\
    \< \sendmessageleft*{\pcbox{\boldsymbol{M_{2}}: \{k_{i},X_{d}\}}} \< \\
        DPAN_{s}\gets Train(X_{d},Dev_{i}) \<\<\\
        \textbf{Store}\ \{k_i,Dev_i,DPAN_s\} \<\<
}
\end{adjustbox}
% }
\end{mdframed}


% change the dpan to algorithm 1.
